Almost Envy-freeness, Envy-rank, and Nash Social Welfare Matchings

Envy-free up to one good (EF1) and envy-free up to any good (EFX) are two well-known extensions of envy-freeness for the case of indivisible items. It is shown that EF1 can always be guaranteed for agents with subadditive valuations. In sharp contrast, it is unknown whether or not an EFX allocation always exists, even for four agents and additive valuations. In addition, the best approximation guarantee for EFX is $(\phi -1) \simeq 0.61$ by Amanitidis et al.. In order to find a middle ground to bridge this gap, in this paper we suggest another fairness criterion, namely envy-freeness up to a random good or EFR, which is weaker than EFX, yet stronger than EF1. For this notion, we provide a polynomial-time $0.73$-approximation allocation algorithm. For our algorithm, we introduce Nash Social Welfare Matching which makes a connection between Nash Social Welfare and envy freeness. We believe Nash Social Welfare Matching will find its applications in future work.

==> files/Improve.tex <==
\section{Improving the Approximation Ratio}
\textcolor{red}{This section is written informally.}

Throughout this section, we show that with a more careful allocation of the goods, we can improve the approximation factor to $3/4$. Indeed, our method is very similar to the previous algorithm, except that some parts of step 1 and step 3 is updated. First, recall the definition of groups $\group_1$, $\group_2$, and $\group_3$ and let $c=8/3$. 

%We define $\group_{1.5}$ as follows:
%\begin{itemize}
%	\item $\group_{1.5}$ contains every agents $i$  in $\group_1$ such that $ 8/3<r_i< 3$ and there exists an agent $j$ in $\group_3$ such that  $$\valu_j(\allocation_i) \geq \valu_j(\allocation_j).$$
%\end{itemize}
%
%Furthermore, let $\group_1 = \group_1 \setminus \group_{1.5}$. Therefore, we now have four different groups $\group_1,\group_{1.5},\group_2,$ and $\group_3$.
%In addition, define group  $\group_{3.5}$ to be a subset of $\group_3$ containing every agent $i$ such that $i$ envies at least one agent in $\group_{1.5}$ with ratio more than $8/3$, i.e.,
%$$
%i \in \group_{3.5} \iff \exists j \in \group_{3.5} \quad \mbox{s.t.} \quad \valu_i(\allocation_j) > 8.3\cdot \valu_i(\allocation_i). 
%$$

After the second step, every agent in $\group_3$ has three items, every agent in $\group_2$ has two items, and every agent in $\group_1$ has  one items. Furthermore, we know that Observation \ref{before_step_3} holds after the second step. For every remaining item $\ite$ we have:
\begin{itemize}
	\item If $i \in \group_1$, $\valu_i(\ite) <  \valu_i(A_i)/c$.
	\item If $i \in \group_2$, $\valu_i(\ite) < \valu_i(A_i)/3$.
	\item If $i \in \group_3$, $\valu_i(\ite) <  \valu_i(A_i)/3$. 
\end{itemize}
A closer look at these conditions reveals that the only condition that prevents our algorithm to be a $3/4$ approximation is the first condition. Now, let $\group_{1.5}$ be a subset of the agents in $\group_1$ that are problematic! An agent in $\group_1$ is problematic, if the following conditions hold:
\begin{itemize}
	\item $1 \leq r_i $.
\end{itemize}

==> files/conclusion.tex <==
\section{Conclusions and Future Directions} 
In this paper, we proposed a new relaxation of envy-freeness, namely envy-freeness up to a random item ($\efr$), which is stronger than $\efo$ but weaker than $\efx$. These two relaxations of envy-freeness have been vastly studied. A simple round-robin algorithm guarantees $\efo$ but it is unknown whether the $\efx$ allocation always exists. In this paper, we studied the approximation algorithms for $\efr$ and $\efx$ when agents have additive valuations. We provide a polynomial-time $0.72$-approximation $\efr$ algorithm and a new $0.61$-approximation $\efx$ algorithm. The first immediate open problem is to improve these approximation factors. For the initial step of our algorithms, we introduce Nash social welfare matching, and our belief is that this technique can be useful to improve the approximations bounds for the other fairness notions. 

The other line of research that we propose is to study almost envy-freeness for the allocation of indivisible chores. Similar to the case of indivisible itmes, a simple round-robin algorithm guarantees $\efo$ allocation for the indivisible chores. However, the same techniques for approximating the $\efx$ allocation of items do not work here, and giving any approximation factor for the $\efx$ allocation of chores is an open problem.

%\textcolor{red}{Some of the paragraphs are pasted here.}
%
%Another important fairness notion is proportionality, introduced by Steinhaus in 1948 \textcolor{red}{ref}. An allocation is called proportional, if the value of assigned bundle to each agent is at least 1/n fraction of his total value for all the goods, where n is the number of agents. Dubins and Spainer in 1961 [21] propose a simple moving-knife algorithm that can guarantee a proportional allocation of a divisible good. However, similar to the envy-freeness, the proportional allocation of indivisible items is not also always possible. Here again, in the embarasing example of two agents with only one item we cannot guarantee proportionality if the item has positive value for both agents.
%
%Conitzer et al. in \textcolor{red}{ref to Fair Public Decision Making} proposed a relaxation of proportionality, called \textit{proportionality up to one item (Prop1)}. It states that every player should be able to get his proportional share if he receives an item outside of his allocation in his favor. Conitzer et al. in \textcolor{red}{ref to Fair Public Decision Making} showed such an allocation always exists. \textcolor{red}{blah [ref]} extended this definition to \textit{proportionality up to any item (PropX)} which states that an agent should be able to get his proportional share if he receives his least favorite item outside of his own allocation. \textcolor{red}{blah [ref]} showes that such an allocation may not exist. We also introduce a new relaxation of proportionality, called \textit{proportionality up to a random item (PropR)} which states that an agent should be able to get his proportional share in expectation if he receives a random item outside of his own allocation. We show such an allocation may not exist. 

==> files/results.tex <==
\begin{example}{A PROPR allocation may not exist.}

\begin{table}[ht]
\centering
\caption{Counter-example for the existence of PROPR}
\begin{tabular}[t]{ccccccc}
\hline
&a&b&c&d&e&f\\
\hline
1&3&0&0&0&0&0\\
2&3&0&0&0&0&0\\
3&3&0&0&0&0&0\\
\hline
\end{tabular}
\end{table}  

According to the pigeon hole principle, in any allocation, at least one of the agents gets at most two items with zero value and does not get item $a$. Without loss of generality, assume that agent 1 is such an agent. In a proportional allocation, $V_1(\allocation_1) \geq 1$. However, we know $V_1(\allocation_1) + \frac{ V_1(\items \setminus \allocation_1)}{ |\items \setminus \allocation_1|} \leq  0 + 3/4 < 1$. Hence, a PROPR allocation does not exist in this example.


\end{example}
